All You Need is RAW: Defending Against Adversarial Attacks with Camera Image Pipelines

Existing neural networks for computer vision tasks are vulnerable to adversarial attacks: adding imperceptible perturbations to the input images can fool these methods to make a false prediction on an image that was correctly predicted without the perturbation. Various defense methods have proposed image-to-image mapping methods, either including these perturbations in the training process or removing them in a preprocessing denoising step. In doing so, existing methods often ignore that the natural RGB images in today's datasets are not captured but, in fact, recovered from RAW color filter array captures that are subject to various degradations in the capture. In this work, we exploit this RAW data distribution as an empirical prior for adversarial defense. Specifically, we proposed a model-agnostic adversarial defensive method, which maps the input RGB images to Bayer RAW space and back to output RGB using a learned camera image signal processing (ISP) pipeline to eliminate potential adversarial patterns. The proposed method acts as an off-the-shelf preprocessing module and, unlike model-specific adversarial training methods, does not require adversarial images to train. As a result, the method generalizes to unseen tasks without additional retraining. Experiments on large-scale datasets (e.g., ImageNet, COCO) for different vision tasks (e.g., classification, semantic segmentation, object detection) validate that the method significantly outperforms existing methods across task domains.

==> bpda.tex <==
In this section, we discuss the modifications of the method to defend against BPDA attack. BPDA and derivative methods rely on building a differentiable proxy for a non-differentiable input transformation method (\ie, obfuscated
gradients) to approximate gradients. In order to tackle such an attack, we modified our transformation algorithm from a determined algorithm to a randomized algorithm so that the adversary cannot build an accurate proxy.

The modifications are shown listed in Algorithm \ref{alg:inf2}; see original Algorithm \ref{alg:inf1}. Specifically, at the inference time, instead of transforming the input image and directly feeding it to the downstream model, we apply our method $N$ times sequentially, where the output of each transformation is the input for the next one. We add small random noise perturbations to the RGB image and Raw Image during each transformation. Here, two randomization effects are introduced: the number of times of applying transformation, $N$, is also random. By introducing sufficient randomization, it is hard to build an accurate proxy to get the precise gradient, and then we can defend against the BPDA attack. Note that the new algorithm only requires modification at the inference stage, whereas the training stage remains the same, hence there is no need to retrain the model. 

\begin{minipage}{0.46\textwidth}
\vspace{-22mm}
\begin{algorithm}[H]
\scriptsize
\captionsetup{font=scriptsize}

\caption{Original Inference Algorithm}\label{alg:inf1}
\begin{algorithmic}[1]

% \hspace*{\algorithmicindent} \textbf{Input} \\
\Require  Input Image $I$, Operator $S, F, G$, Hyper-parameter $\omega$
% \Ensure $y = x^n$
\vspace{2mm}
\State $Raw \gets F(I)$
\State $I \gets \omega * G(Raw) + (1 - \omega) * S(Raw)$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
\scriptsize
\captionsetup{font=scriptsize}
\caption{Modified Inference Algorithm}\label{alg:inf2}
\begin{algorithmic}[1]

% \hspace*{\algorithmicindent} \textbf{Input} \\
\Require  Input Image $I$, Operator $S, F, G$, Hyper-parameter $\omega$
% \Ensure $y = x^n$
\vspace{2mm}
\State $N \gets random(0,20)$
\State $i \gets 0$
\While{$i \neq N$}
    \State $n_I \gets Gaussian(\mu = 0, \sigma = 0.05)$
    \State $n_{Raw} \gets Gaussian(\mu = 0, \sigma = 0.05)$  
    \State $Raw \gets F(I + n_I)$
    \State $Raw \gets Raw + n_{Raw}$
    \State $I \gets \omega * G(Raw) + (1 - \omega) * S(Raw)$
    \State $i\gets i + 1$
    
\EndWhile
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{2mm}

The performance of the defense against BPDA is shown in Table~\ref{tbl:BPDA}. Specifically, the proposed modification improves the defending accuracy from 14.28 to 38.85. Also, compared to the baseline input transformation methods, the proposed method is the only method that shows robustness to the BPDA attack. We also compared the performance of the proposed method with and without modification for all other attacks in the same Table~\ref{tbl:withwithout}, and found that the defense performances under other attacks decrease slightly after introducing the modification. In other words, the modification significantly increase the robustness of the proposed method under the BPDA attack, at the cost of slightly decreasing the defense performance under other attacks. Note that the relative ranking of the proposed defense method versus baseline defense methods remains the same, with the proposed defense method outperforming baselines with a large margin both before and after the modification.

\begin{table}[]
	% \begin{center}
		\vspace{0mm}
		\captionsetup{font=scriptsize}
		\begin{minipage}{0.71\linewidth}
			\begin{adjustbox}{width=1.4\linewidth}
				{\small
					\addtolength{\tabcolsep}{0pt}
					% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
					\begin{tabular}{l|cccc}
						\hline
						\hline
						Defense Method &  JPEG-Defense & TVM & Randomized Resizing \& Padding & Pixel-Deflection \\
						%\hline
						% \hline
						 & 0.08 & 6.39 & 2.66  & 1.87 
						 \vspace{2mm}
						 \\ 
						\hline
						 &  ComDefend & HGD & Proposed Method (Unmodified) & Proposed Method (modified)\\
						%\hline
						% \hline
						 & 0.03 & 0.03 & 14.28 & 38.85
						 \\ 
						  \hline
						  \hline
					\end{tabular}\\
				}
			\end{adjustbox}
		\end{minipage}
		\vspace{1mm}
		 \caption{%\textbf{Evaluation of robustness of Pipeline:} 
		 \textbf{Quantitative comparison with baseline input-transformation defense methods under BPDA attack:} The proposed modification improves the defending accuracy from 14.28 to 38.85, and the resulting method significantly outperforms the baselines.}
		  \label{tbl:BPDA}
	% \end{center}
	\vspace{-10mm}
\end{table}


\begin{table*}[]
	% \begin{center}
		\vspace{-4mm}
		\captionsetup{font=footnotesize}
		\begin{minipage}{0.71\linewidth}
			\begin{adjustbox}{width=1.4\linewidth}
				{\small
					\addtolength{\tabcolsep}{0pt}
					% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
					\begin{tabular}{l|cccccccccccc}
						\hline
						\hline
						 & \multicolumn{2}{c}{FSGM} & \multicolumn{2}{c}{PGD} & \multicolumn{2}{c}{BIM} & \multicolumn{2}{c}{DeepFool} & \multicolumn{2}{c}{C\&W}  & NewtonFool & BPDA\\
						 & $2/255\uparrow$ & $4/255\uparrow$ &$2/255\uparrow$ & $4/255\uparrow$ & $2/255\uparrow$ & $4/255\uparrow$ & $L_{\infty}\uparrow$ & $L_{2}\uparrow$ & $L_{\infty}\uparrow$ & $L_{2}\uparrow$  &  $L_{\infty}\uparrow$ & $L_{\infty}\uparrow$
						\\
						\hline
						 & \multicolumn{11}{c}{\textbf{ResNet-101}}
						\\[2pt]		
						% \hline
						% \hline
					     JPEG-Defense\cite{JPEG_eval} & 33.14 & 20.71 &	45.19 & 21.74 &	36.78  & 8.5  &	53.16 & 45.69 &	59.06 & 52.01 &	24.65 & 0.08\\ 
						% \hline
						 TVM\cite{guo2017countering}  & 43.75 & 40.02 &	45.46 & 44.35 &	44.86 & 41.93 &	47.69 & 39.89 &	45.51 & 40.44 &	22.6 & 6.39
						 \\ 
						% \hline
						Randomized Resizing \& Padding\cite{xie2017mitigating} & 45.21 & 34.97 &	45.38 &  27.75 &	40.04 & 18.04  &	73.06 &62.47 &	66.53 &  59.87 &	27.93 & 2.66
						   \\ 
						% \hline
						HGD \cite{liao2018defense}& 54.75 & 43.85 &	55.26 & 50.05 &	56.74 &  48.61  &	64.34 & 58.13 &	59.98 & 52.88 &	27.70 &0.03
								\\		
						% \hline
						Pixel-Deflection\cite{prakash2018deflecting} & 54.56 & 35.14 & 60.68 & 34.86 &	58.71 & 41.91  &	75.97 & 64.13 & 66.29 & 60.91 &	28.81 & 1.87
						 \\ 
						% \hline
						ComDefend\cite{jia2019comdefend} & 48.21 & 36.51 &	53.28 & 48.38 &	51.39 &  42.01  &	63.68 & 55.62 &	58.53 & 50.38 &	26.46 & 0.03
								\\		
						Proposed Method w/o modification   & 66.02 & 58.85  & 68.34  & 66.17 &	66.91 & 63.01 &	72.04 & 63.52 &	71.40 & 67.33  &	40.96 & 14.28
						\\
						% \vspace{2mm}
						Proposed Method w/ modification   & 61.87 & 54.42  & 63.79  & 59.03 &	61.29 & 57.35 &	68.80 & 56.42 &	68.13 & 61.65  &	35.88 & 38.85
						\\
						\hline
						 & \multicolumn{11}{c}{\textbf{InceptionV3}}
						\\[2pt]	
						JPEG-Defense\cite{JPEG_eval} & 31.97 & 20.25 & 43.34 & 21.15 &  34.68 & 8.55& 51.20 & 43.49 & 55.00 & 50.39 & 24.06 & 0.12
						\\ 
						% \hline
						TVM\cite{guo2017countering}  & 42.47 & 37.23 & 42.75 & 41.61 & 42.80 & 39.71 & 45.21  & 37.39  & 43.27 & 37.51 & 23.05 & 4.58

						 \\ 
						% \hline
						Randomized Resizing \& Padding\cite{xie2017mitigating} & 41.86 & 34.49  & 43.41 & 25.60 & 39.42 & 16.62  & 70.24 & 58.65 & 63.24  & 55.62 & 27.55 & 2.09

						   \\ 
						   
                        HGD \cite{liao2018defense}& 52.83 & 40.99  & 50.35 & 47.62 & 56.02 & 47.78  & 60.33 & 56.61 & 59.55  & 52.0 & 26.84 & 0.03 
                        \\
						% \hline
						Pixel-Deflection\cite{prakash2018deflecting} & 51.42  & 34.27  & 56.13   & 32.49  & 56.18  & 39.13   & 71.16  & 61.58  & 	61.94  & 57.58  & 28.01 & 1.56

						 \\ 
						% \hline
						ComDefend\cite{jia2019comdefend} & 47.00 & 35.34  & 49.99  & 46.15 & 48.74  & 39.58  & 60.01  & 52.47  & 55.85  & 47.70  & 25.44 & 0.03

								\\							
						% \hline
						Proposed Method w/o modification   & 63.03  & 	56.34  & 65.69  & 	63.03  & 64.77  & 	59.49   & 69.25   & 60.04   & 66.97  & 64.69  & 38.01 & 12.11 

								\\				
						% \hline
						Proposed Method w/ modification   & 59.89  & 	53.02  & 61.15  & 	59.44  & 58.07  & 	57.92   & 66.48   & 55.84   & 61.25  & 60.30  & 35.63 & 36.43 

						  \\ 
						  \hline
						  \hline
						  
					\end{tabular}\\
				}
			\end{adjustbox}
		\end{minipage}
		\vspace{1mm}
		\captionsetup{font=scriptsize,labelfont=scriptsize}
		\caption{{\textbf{Quantitative Comparisons for the proposed method w/ and w/o modification for BPDA.} The modification significantly increase the robustness of the proposed method under BPDA attack, at the cost of slightly decreasing the defense performance under other attacks. The relative ranking of the proposed defense method versus baseline defense methods remains the same, with the proposed defense method outperforming baselines with a large margin both before and after modification.}}
		 \label{tbl:withwithout}
		 
	% \end{center}
	\vspace{-5mm}
\end{table*}
% \begin{algorithm}
% \scriptsize
% \captionsetup{font=scriptsize}
% \caption{Modified Inference Algorithm}\label{alg:cap}
% \begin{algorithmic}

% % \hspace*{\algorithmicindent} \textbf{Input} \\
% \Require  Image $I$, Operator $S, F, G$
% % \Ensure $y = x^n$
% \State $N \gets random(0,20)$
% \State $i \gets 0$
% \While{$i \neq N$}
%     \State $noise1 \gets Gaussian(\mu = 0, \sigma = 0.05)$
%     \State $noise2 \gets Gaussian(\mu = 0, \sigma = 0.05)$  
%     \State $Raw \gets F(I + noise1)$
%     \State $Raw \gets Raw + noise2)$
%     \State $I \gets \omega * G(Raw) + (1 - \omega) * S(Raw)$
%     \State $i\gets i + 1)$
    
% \EndWhile
% \end{algorithmic}
% \end{algorithm}



==> defense_baselines.tex <==
In this section, we provide additional detail on the baseline adversarial defense methods used in our experiment. These baselines methods are state-of-the-art input-transformation defense methods with released code.

\begin{enumerate}

\item{\textbf{JPEG-Defense\cite{JPEG_eval}:}} The JPEG-Defense method is a defense method based on input transformation. The intuition behind the method is that the compression process may remove high-frequency adversarial perturbations. A hyper-parameter of this method is the compression ratio, which affects the adversarial defense accuracy. A high compression ratio results in high image quality but also leads to less removal of adversarial perturbations. In our experiment, we set the compression ratio to 75\%, which is consistent with the setting proposed in \cite{JPEG_eval}.

\vspace{2mm}
\item{\textbf{ComDefend\cite{jia2019comdefend}:}} Similar to JPEG-Defense, ComDefend also aims to remove unnecessary details of the input image through compression. But unlike JPEG compression, ComDefend learns an auto-encoder to compress and reconstruct the image. Specifically, an encoder maps the input image to a compressed latent space, which is then fed into the decoder for reconstruction.

\vspace{2mm}
\item{\textbf{TVM\cite{guo2017countering}:}}  The method works by randomly selecting a small set of pixels and reconstructing the "simplest" image that is consistent with the selected pixels. The reconstructed image is intended to be "simple" so that it does not contain adversarial perturbations. The ``simple'' is defined in terms of the total variation. A hyperparameter of this method is the number of pixels to be selected. Selecting a large portion of pixels keeps more image details but also keeps more adversarial perturbations. In our experiment, we tune the hyperparameter to achieve the best performance.

\vspace{2mm}
\item{\textbf{Randomized Resizing \& Padding \cite{xie2017mitigating}:}} The method aims to mitigate the effect of adversarial perturbations through randomization. Given an input image, two randomization operations are performed. In particular, the method first randomly resizes the input image. Then, it randomly pads zeros around the input images. 

\vspace{2mm}
\item{\textbf{Pixel-Deflection\cite{prakash2018deflecting}:}} The method works by forcing the image to match natural image statistics. In doing so, the algorithm locally corrupts the image by redistributing pixel values by pixel deflection. Then, a subsequent wavelet-based denoising operation softens this corruption. 


 
\end{enumerate}


==> proxyattack.tex <==
\begin{table*}[h]
	% \begin{center}
		\vspace{-2mm}
		\begin{minipage}{0.71\linewidth}
			\begin{adjustbox}{width=1.4\linewidth}
				{\small
					\addtolength{\tabcolsep}{0pt}
					% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
					\begin{tabular}{l|cccccc}
						\hline
						\hline
						 & JPEG-Defense\cite{JPEG_eval} & TVM\cite{guo2017countering}  & Randomized Resizing \& Padding\cite{xie2017mitigating} & Pixel-Deflection\cite{prakash2018deflecting}  & ComDefend\cite{jia2019comdefend} & Proposed Method  
						 \\ 
						 \hline
						% \hline
						Proxy Attack & 5.33 & 6.28&	6.91  &	6.03 &  5.87  &	6.72
						\\
						\hline
						\hline
						  
					\end{tabular}\\
				}
			\end{adjustbox}
		\end{minipage}
		\vspace{-2mm}
		 \large{ \caption{We evaluate the proposed defense method against proxy attack~\cite{phan2021adversarial}, where we build a differentiable proxy for the non-differential part of preprocessing pipelines and expose the gradient to the adversary. No existing input-transformation-based defense method can survive such an attack.}  \label{tbl:proxy}}
	% \end{center}
	\vspace{0mm}
\end{table*}


The last section considers the super-white box attack setting where an adversary has full access to both preprocessing modules and target models. Here, we consider a black-box setting where an adversary has access to neither preprocessing modules nor target models. But, given input to a target model, the corresponding output is exposed. An adversary can train a differentiable proxy model with the collected input-output pairs, mimicking the target model's behaviors. This practice allows the adversary to generate adversarial samples based on the gradients of the differentiable proxy model~\cite{phan2021adversarial}. It is important to note, regardless of whether the preprocessing modules are deterministic or not, the proxy-based attack works effectively in both cases. For the non-deterministic ones, the adversary can leverage Expectation over Transformation (EOT) \cite{athalye2018obfuscated} strategy to counter the randomness in the preprocessing pipeline. 

We evaluate the defense performance of all competing methods against such a proxy attack. Specifically, we train proxy models separately for all competing methods, including the $S$ module of our approach, the JPEG compression module~\cite{JPEG_eval}, the TVM module~\cite{guo2017countering}, the Randomized Resizing \& Padding module~\cite{xie2017mitigating}, and the Pixel-Deflection module~\cite{prakash2018deflecting}. For each preprocessing module, we perform FSGM-based attacks according to the gradients of the corresponding proxy model. As shown in table \ref{tbl:proxy}, all existing input-transformation-based defense methods suffer from proxy attacks. 

Note that our specific application of the proxy attack requires here a tap-out of the input image and the defense output which could be prohibited by encrypting data between these stages in a hardware implementation.


% In the last section, we consider the super-white attack setting where an adversary has full access to both preprocessing modules and target models. and therefore can calculate the gradient of differentiable part of the preprocessing module to construct a strong attack. In this section, we consider the case where we have a "smarter" adversary. That is, for the non-differentiable part of preprocessing module, the adversary would build a differentiable proxy by training an image-to-image model (i.e., auto-encoder) using corresponding input-output pairs. This practice allows the adversary to obtain the approximate gradient using the differentiable proxy, and then construct a stronger attack than the super-white attack where only the differentiable preprocessing part is exploited. Note that the idea of building a differentiable proxy can work both for the deterministic preprocessing method and non-deterministic preprocessing module, where the adversary can exploit Expectation over Transformation (EOT) \cite{athalye2018obfuscated} strategy to counter the randomness in the preprocessing pipeline. 

% We evaluate the defense performance of the prosed method and baselines against such a proxy attack. Specifically, we train proxy models for the $S$ module as well as for all the non-differential modules baseline methods (the JPEG compression module in \cite{JPEG_eval}, the TVM module in \cite{guo2017countering}, the Randomized Resizing \& Padding module in \cite{xie2017mitigating}, and the Pixel-Deflection module in \cite{prakash2018deflecting}). We then perform FSGM attack using the approximate gradient of the preprocessing module. As shown in table \ref{tbl:proxy}, all existing input transformation defense method fail to survive such an attack.  We leave addressing such a proxy attack for future work.



==> supp_Qualitative_result.tex <==
\begin{figure*}[]
	\centering
	\resizebox{\linewidth}{!}{
	\renewcommand{\arraystretch}{0.5}
	\begin{tabular}{ccccccccccc}
	
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000005_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000005_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000005_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000005_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000005_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000005_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000005_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000005_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000005_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000005_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000005_recons_weighted.png} 		
		\\[.2cm]

		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000031_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000031_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000031_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000031_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000031_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000031_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000031_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000031_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000031_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000031_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000031_recons_weighted.png} 	
		\\[.2cm]
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000081_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000081_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000081_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000081_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000081_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000081_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000081_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000081_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000081_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000081_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000081_recons_weighted.png} 	
		\\[.2cm]	
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000021_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000021_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000021_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000021_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000021_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000021_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000021_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000021_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000021_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000021_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000021_recons_weighted.png} 	
		\\[.2cm]
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000085_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000085_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000085_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000085_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000085_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000085_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000085_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000085_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000085_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000085_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000085_recons_weighted.png} 	
		\\[.2cm]			

		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000087_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000087_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000087_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000087_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000087_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000087_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000087_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000087_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000087_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000087_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000087_recons_weighted.png} 	
		\\[.2cm]	
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000065_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000065_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000065_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000065_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000065_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000065_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000065_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000065_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000065_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000065_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000065_recons_weighted.png} 	
		\\[.2cm]
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000030_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000030_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000030_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000030_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000030_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000030_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000030_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000030_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000030_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000030_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000030_recons_weighted.png} 	
		\\[.2cm]	

		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000036_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000036_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000036_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000036_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000036_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000036_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000036_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000036_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000036_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000036_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000036_recons_weighted.png} 	
		\\[.2cm]	
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000022_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000022_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000022_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000022_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000022_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000022_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000022_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000022_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000022_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000022_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000022_recons_weighted.png} 		
		\\[.2cm]		
		
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000006_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000006_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000006_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000006_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000006_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000006_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000006_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000006_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000006_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000006_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000006_recons_weighted.png} 	
		\\[.2cm]			

		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000051_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000051_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000051_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000051_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000051_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000051_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000051_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000051_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000051_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000051_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000051_recons_weighted.png} 	
		\\[.2cm]	

		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000011_original_images.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000011_adv_images.png}&
		\includegraphics[width=0.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000011_perturbation.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_JPEG_png/000011_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_TVM_png/000011_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_ResizePad_png/000011_recons_weighted.png} & 
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_pixel_deflection_png/000011_recons_weighted.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_comdefend_png/000011_recons_weighted.png} &	
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000011_recons_deep_isp.png}&
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000011_recons_isp.png} &
		\includegraphics[width=.35\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{figs/results/visual_our_png/000011_recons_weighted.png} 	
		\\[.2cm]
		
		
		
		
		
		\centering
		{ \huge{Clean Image}}&
		{ \huge{Adversarial Image}}&
		{ \huge{Perturbation}}&		
		{ \huge{JPEG-Defense\cite{JPEG_eval}}} &
		{ \huge{TVM\cite{guo2017countering} }} &
		{ \huge{Resizing \& Padding\cite{xie2017mitigating} }} &
		{ \huge{Pixel-Deflection\cite{prakash2018deflecting}}} &
		{ \huge{ComDefend\cite{jia2019comdefend}}} & 
		{ \huge{Operator $G$}}&
		{ \huge{Operator $S$}} &
		{ \huge{Proposed Method}} 		
		\\		
	\end{tabular} 
	}
	\vspace{-2mm}
    \caption{\footnotesize{Qualitative comparison of the proposed method along with both $G$ and $S$ operators against state-of-the-art defense methods on the ImageNet dataset, see text.}}
    \label{fig:more_qualitative} 
    % \caption{\textbf{Qualitative Examples.} We show qualitative examples of baseline defense methods and the proposed method, including the operator outputs of $G$ and $S$. }
    \vspace{-2mm}
\end{figure*}

In this section, we provide additional qualitative results from the proposed methods and state-of-the-art defense baselines. For input-transformation-based adversarial defense methods, a balance between transformation fidelity and adversarial patterns removal is essential. A higher transformation fidelity indicates more details of the original image are kept, including adversarial patterns. In contrast, radical pattern removal could result in a severe loss of detail. This balance is achieved by a simple weighted sum between the $G$ and $S$ operator in our method. The $S$ operator is designed for faithfully reconstructing high-frequency details, while the $G$ operator is trained to mitigate adversarial patterns. As shown in Figure \ref{fig:more_qualitative}, our approach offers better transformation fidelity than Comdefend, TVM, Pixel Deflection, and Resizing \& Padding methods. Even though the JPEG-Defense method keeps more high-frequency details than the ones offered by our approach, it suffers from removing adversarial patterns, resulting in the worst performance among all compared methods.

% In this section, we show more qualitative results from the proposed methods and state-of-the-art defense baselines in figure \ref{fig:more_qualitative}. For the adversarial defense method based on input transformation, a good balance between transformation fidelity and adversarial patterns removal is required. A high fidelity means the transformed image keeps the same details as the input image. However,  a 100\% fidelity would lead to 0\% defense accuracy, as all adversarial patterns are kept. On the contrary, radical pattern mitigation would remove most of the adversarial patterns, but at the same time, may result in a severe loss of details that help the decision-making of downstream models.  Thus, a good balance between transformation fidelity and adversarial patterns removal is required. In our method, the G operator learns to mitigate the adversarial pattern, while the S operator can faithfully reconstruct high-frequency details.  Combining them in a weighted sum manner allows us to achieve such a good balance. As the figure \ref{fig:more_qualitative} shows, compared to the baseline method, we achieve better transformation fidelity than Comdefend, TVM, Pixel Deflection, Resizing \& Padding. Meanwhile, JPEG-Defense keeps too many details from the input image, resulting in limited removal adversarial pattern and thus the worst performance among all the methods.



==> supp_SO.tex <==
The $S$ operator offers the functionality of a conventional (hardware) ISP pipeline using a sequence of cascaded sub-modules. In particular, the proposed $S$ operator consists of the following components: Bayer Demosaicking, color balancing, white balancing, contrast enhancement, Gamma adjustment, and colorspace conversion sub-modules. We provide the implementation details of each sub-module below:


% In this section, we provide more details regarding the $S$ operator of synthetic software ISP used in the proposed approach. Our pipeline consists of six main modules: Bayer Demosaicking module, Color Balance module, White Balance module, Contrast Improvement module, Gamma Adjustment module, and Colorspace Conversion module. Details of each module are illustrated below

\begin{enumerate}

\item{\textbf{Bayer Demosaicking}:} As discussed in the main manuscript, a color filter array (CFA) sits on a matrix of small potential wells. When light passes through the CFA layer, a mosaic pattern of the three stimulus RGB colors is generated, called RAW image. A Bayer pattern mosaic is the most commonly used one, alternating R-G-G-B $2 \times 2$ superpixels. To reconstruct trichromatic intensity values from a RAW image, a demosaicking algorithm is required. In our implementation, we use the DDFaPD demosaicking algorithm \cite{menon2006demosaicing} offered by the Python colour-demosaicing library.

% In a digital camera, a color filter array (CFA) is placed in front of an image sensor to record specific wavelengths of light on different photosite, resulting in the RAW captures with a Bayer mosaic (alternating R-G-G-B $2 \times 2$ color filter array). Trichromatic RGB values are reconstructed from RAW captures, for example by interpolation~\cite{zhang2011color}.  In our pipeline, we use DDFaPD demosaick algorithm \cite{menon2006demosaicing} implemented in Python colour-demosaicing library.
\vspace{2mm}
\item{\textbf{Color Balance }} The purpose of color balancing is to recover the color characteristics of the original scene. We achieve the color balancing by using the SimpleColorBalance \cite{limare2011simplest} algorithm, which is adopted from the OpenCV library. 

% The color balancing step aims to estimate the sensor's R, G, B color filter responses to lighting and adjust colors accordingly. We adopt the color balancing method from the OpenCV library, which implements the SimpleColorBalance \cite{limare2011simplest} algorithm based illumination estimation.

\vspace{2mm}
\item{\textbf{White Balance }:} We further adjust the color temperatures of RGB images with a white balance method to make the color look more natural. We use a white balancing method provided by the OpenCV library, mainly based on the White Patch algorithm and Gray World algorithm~\cite{rizzi2002color}.

\vspace{2mm}
\item{\textbf{Contrast Enhancement}} Contrast plays a critical role in separating the dark and bright areas of an image. An improvement in contrast increases this separation, making objects more distinguishable. In our pipeline, the Contrast Limited Adaptive Histogram Equalization(CLAHE) algorithm \cite{reza2004realization} is leveraged for contrast enhancement.

% Contrast improvement enhance the perceptibility of objects in the scene by improving the brightness difference between objects and their backgrounds. In our pipeline, we use the Contrast Limited Adaptive Histogram Equalization(CLAHE) algorithm \cite{reza2004realization}.

\vspace{2mm}
\item{\textbf{Gamma Adjustment}:} In this step, we use a non-linear Gamma correction function to adjust the image luminance (\ie, brightness level). In our pipeline, we use the OpenCV's gamma correction algorithm \cite{huang2012efficient}.

% Gamma curve is applied to the target image for modifying brightness and achieving more appealing details. In our pipeline, we use the default gamma correction algorithm \cite{huang2012efficient} from the OpenCV library.

\vspace{2mm}
\item{\textbf{Colorspace Conversion}:} Pixel values are converted to a specific colorspace (e.g., to sRGB) before compression (e.g. to jpg), storage, or further processing. 

\end{enumerate}

\noindent The $F$ operator is a small learned encoder-decoder network to map an RGB image to its intermediate RAW measurements. The details of network architecture are shown below in Table \ref{tab:RGB2RAW}

\begin{table}[]
    
	\centering
	\fontsize{9}{12}\selectfont   
	\vspace{-7mm}
	\caption{Architecture description of the $F$ Operator.}
	%\vspace{-2mm}
	\begin{tabular}{p{0.10\textwidth}p{0.28\textwidth}p{0.22\textwidth}
	p{0.22\textwidth}p{0.08\textwidth}}
		\toprule
% 		\cmidrule(lr){1-5}
		Layer & Type & In-Channel & Out-Channel & Kernel  \cr
		\cmidrule(lr){1-5}
		1st & Conv+Relu & 3 & 32 & 3$\times$3   \cr
		2nd & Conv+Relu & 32 & 64 & 3$\times$3   \cr
		3rd & Conv+Relu & 64 & 128 & 3$\times$3   \cr
		4th & UpConv+Relu & 128 & 64 & 3$\times$3   \cr
		5th & UpConv+Relu & 64 & 32 & 3$\times$3   \cr
		6th & UpConv+Sigmoid & 32 & 1 & 3$\times$3   \cr
		\bottomrule
	\end{tabular}\vspace{0cm}
	\label{tab:RGB2RAW}
	\vspace{-8mm}
\end{table}


% \begin{table}[]
% \vspace{-0mm}
% \begin{center}
% \begin{minipage}{0.9\linewidth}
%  \begin{adjustbox}{width=1\linewidth}
%  \fontsize{6}{9}\selectfont   
% 	\begin{tabular}{p{0.06\textwidth}p{0.2\textwidth}p{0.16\textwidth}
% 	p{0.16\textwidth}p{0.06\textwidth}}
% 		\toprule
% % 		\cmidrule(lr){1-5}
% 		Layer & Type & In-Channel & Out-Channel & Kernel  \cr
% 		\cmidrule(lr){1-5}
% 		1st & Conv+Relu & 3 & 32 & 3$\times$3   \cr
% 		2nd & Conv+Relu & 32 & 64 & 3$\times$3   \cr
% 		3rd & Conv+Relu & 64 & 128 & 3$\times$3   \cr
% 		4th & UpConv+Relu & 128 & 64 & 3$\times$3   \cr
% 		5th & UpConv+Relu & 64 & 32 & 3$\times$3   \cr
% 		6th & UpConv+Sigmoid & 32 & 1 & 3$\times$3   \cr
% 		\bottomrule
% 	\end{tabular}\vspace{0cm}
% \end{adjustbox}
% \end{minipage}
% \hfill
% \begin{minipage}{0.08\linewidth}
% %\vspace{3mm}
% \captionsetup{font=footnotesize,labelfont=footnotesize}
% \caption{
% {\textbf{Architecture description of the $F$ Operator}
% % : The $F$ operator is a small learned encoder-decoder network to map an RGB image to its intermediate RAW measurements.
% }
% }
% \label{tab:RGB2RAW}
% \end{minipage}
% \end{center}
% \vspace{-10mm}
% \end{table}

==> supp_attack.tex <==
In this section, we provide formal definitions for the attack algorithms which are used for validation of the proposed defense method. 
\vspace{2mm}

\begin{enumerate}
     

\item{\textbf{FSGM:}} The FSGM~\cite{goodfellow2015explaining} is an attack method that, for each pixel, determines in which direction the pixel intensity should be moved according to the gradient of the loss function. Mathematically, the adversarial perturbation $\delta$ is defined by FGSM as:
% method designs the adversarial pattern by exploiting the gradient of the input image. Specifically, it determines the direction to modify each pixel value based on the gradient with respect to the loss function. Mathematically, given a clean input image x and corresponding ground truth label y, the attack method generate the adversarial perturbation $\delta$ by:

\begin{align*}
	\delta = \epsilon \cdot \text{sign}(\nabla_{x} L(x,y)),
\end{align*}
where $\epsilon$ is the maximum perturbation allowed for an attack, which is commonly sufficiently small for undetectable; $x$ and $y$ are a benign image and the corresponding ground truth label, respectively.
\vspace{2mm}

\item{\textbf{BIM:}} The BIM~\cite{kurakin2017adversarial} attack is an enhanced version of FGSM. Instead of taking one single step of size $\epsilon$, it iteratively searches for an optimal perturbation with multiple smaller steps $\alpha$. Then, the obtained perturbation is clipped by the predefined $\epsilon$. Formally, BIM is defined as
% attack improves FSGM by iteratively finding the optimal perturbation within the $\epsilon$ neighborhood of the input image.Specifically, given a clean input image x and corresponding ground truth label y. With the initial $x_0 = x$, the method iteratively find $x_i$ by

\begin{align*}
	x_i = \text{clip}_{\epsilon,x} (x_{i-1} + \alpha \cdot \text{sign}(\nabla_{x} L(x,y)) ),
\end{align*}
where $x_0 = x$. The number of iteration used is a hyperparameter, and more iterations typically lead to a stronger attack. 
\vspace{2mm}

\item{\textbf{PGD:}} Similar to the BIM attack, the PGD~\cite{madry2019deep} attack interatively optimzes the adversarial examples generated. With the initial $x_0 = x$, the method iteratively find $x_i$ by:

\begin{equation}
x^{i}=\Pi_{x+S}(x^{i-1}+\alpha\cdot \text{sign}(\nabla_x L(f_{\theta}(x^{i-1}),y))) ,
\end{equation}
where $\Pi_{x+S}$ denotes projecting perturbations into the set $S$. We refer the reader to \cite{madry2019deep} for additional details. The scalar $\alpha$ is the step size used in each iteration and $\epsilon$ denotes the maximum perturbation allowed. 
%\bd{Bo: not very clear to me}%


 \vspace{2mm}
 
\item{\textbf{DeepFool:}} Similar to BIM and PGD, the DeepFool~\cite{moosavidezfooli2016deepfool} attack generates adversarial perturbations iteratively, intending to obtain the perturbation with minimal distortion. Specifically, it finds the closest decision boundary by multiple linearizations of the classifier and then generates the perturbations based on the decision boundary.

\vspace{2mm}

\item{\textbf{C\&W:} The C\&W~\cite{carlini2017evaluating} attack is an optimization-based attack method, which generates the adversarial perturbations by solving the following problem

% The CW~\cite{carlini2017evaluating} attack is an optimization-based attack method. Given a clean input image x and corresponding ground truth label y, the attack algorithm finds the perturbation $\delta$ by:

\begin{align}
	& \min \ \ \ \ \ \ ||\delta||_p + c \cdot f(x+\delta) \nonumber\\ 
	& s.t.  \ \ \ \ \ \  x+\delta \in [0, 1]^n
\end{align}
\noindent where $f$ is a objective function that is designed to mislead the example $x$ to be misclassified; $||\cdot||_p$ denotes $l_p$ norm; and $c$ is a constant, estimated by binary search. 

\vspace{2mm}
\item{\textbf{NewtonFool:}} NewtonFool \cite{jang2017objective} attack is essentially a variant of DeepFool attack. In contrast to DeepFool generating perturbations based on linearization approximation, the NewtonFool is based on nonlinear constraints, allowing for a significantly faster generation of adversarial patterns. Hence, with the same time budget, more iterations can be performed, resulting in stronger attacks.


% NewtonFool~\cite{jang2017objective} attack is essentially a variant of DeepFool attack, which can generate even stronger adversarial patterns. Similar to DeepFool, it aims to find a strong adversarial example in the minimum neighborhood of input image through an iterative process. It differs from DeepFool that Newton’s method for solving nonlinear constraints. This practice allows for a significantly faster generation of adversarial patterns. With the same time constraints budget, more iteration can be performed, resulting in stronger attack.

\vspace{2mm}
\item{\textbf{DAG:}}}
The DAG~\cite{xie2017adversarial} attack is designed to attack semantic segmentation and object detection models. Essentially, it is similar to optimization-based classification attacks, generating adversarial perturbation by solving the following problem:
\begin{equation}
\label{eq:DAG}
    \forall n, {\arg\max_c\left\{f_c\!\left(\mathbf{X}+\mathbf{r},t_n\right)\right\}}\neq{l_n},
\end{equation}
where $X$ is an image which contains $N$ recognition targets ${\mathcal{T}}={\left\{t_1,t_2,\ldots,t_N\right\}}$; ${\mathcal{L}}={\left\{l_1,l_2,\ldots,l_n\right\}}$ is the ground-truth class labels of ${\mathcal{T}}$, \ie, $l_n$ is the ground-truth label of $t_n$; ${\mathbf{f}\!\left(\mathbf{X},t_n\right)}\in{\mathbb{R}^C}$
denote the classification score vector on the $n$-th recognition target; $\mathbf{r}$ denotes an adversarial perturbation to be estimated.

The form of ${\mathcal{T}}$ is defined based on a specific task. For the image classification task, ${\mathcal{T}}$ only contains one element, \ie, the entire image. ${\mathcal{T}}$ becomes all pixels for semantic segmentation tasks, while it becomes all proposals for object detection tasks.

\vspace{1mm}
Intuitively, the goal of the Eq.~\ref{eq:DAG} is to make the predictions of all targets incorrect by estimating an adversarial perturbation $\mathbf{r}$. In doing so, adversarial labels ${\mathcal{L}'}={\left\{l'_1,l'_2,\ldots,l'_n\right\}}\quad \forall i, l_i \neq l'_i$ are required, which are generated by randomly sampling from other incorrect classes.  Under this setting, the loss function covering all targets can be written as
\begin{equation}
\label{Eqn:LossFunction}
{L\!\left(\mathbf{X},\mathcal{T},\mathcal{L},\mathcal{L}'\right)}=
    {{\sum_{n=1}^N}\left[{f}_{l_n}\!\left(\mathbf{X},t_n\right)-{f}_{l_n'}\!\left(\mathbf{X},t_n\right)\right]}.
\end{equation}
Minimizing $L$ can be achieved by making every target an incorrect prediction, \ie, suppressing the confidence of the original correct class $f_{l_n}\!\left(\mathbf{X}+\mathrm{r},t_n\right)$,
while increasing  the confidence of desired (adversarial) incorrect class $f_{l'_n}\!\left(\mathbf{X}+\mathrm{r},t_n\right)$).


% Specifically, Let $\mathbf{X}$ be an image which contains $N$ pixels ${\mathcal{T}}={\left\{t_1,t_2,\ldots,t_N\right\}}$ and corresponding  ground-truth class labels ${\mathcal{L}}={\left\{l_1,l_2,\ldots,l_n\right\}}$. Let $C$ denotes the number of class. Given a semantic segmentation model $f$,
% let ${\mathbf{f}\!\left(\mathbf{X},t_n\right)}\in{\mathbb{R}^C}$
% denote the classification score of pixel $t_n$ over each class. The adversarial attack aims to fool the model $f$ so that it predicts wrong label for all pixels
% {\em i.e.}, $\forall n$, ${\arg\max_c\left\{f_c\!\left(\mathbf{X}+\mathbf{r},t_n\right)\right\}}\neq{l_n}$. To achieve this goal, the algorithm crafts a wrong label set by randomly sampled from incorrect classes, which is denoted as ${\mathcal{L}'}={\left\{l'_1,l'_2,\ldots,l'_n\right\}}$, where $\forall i, l_i \neq l'_i$ The algorithm then minimize the loss $L$ that drive each every pixel to be incorrectly predicted ({\em i.e.}, suppressing the confidence of the original correct class $f_{l_n}\!\left(\mathbf{X}+\mathrm{r},t_n\right)$,
% while increasing  the confidence of desired (adversarial) incorrect class $f_{l'_n}\!\left(\mathbf{X}+\mathrm{r},t_n\right)$)

% DAG~\cite{xie2017adversarial} attack is designed to attack semantic segmentation models. Specifically, Let $\mathbf{X}$ be an image which contains $N$ pixels ${\mathcal{T}}={\left\{t_1,t_2,\ldots,t_N\right\}}$ and corresponding  ground-truth class labels ${\mathcal{L}}={\left\{l_1,l_2,\ldots,l_n\right\}}$. Let $C$ denotes the number of class. Given a semantic segmentation model $f$,
% let ${\mathbf{f}\!\left(\mathbf{X},t_n\right)}\in{\mathbb{R}^C}$
% denote the classification score of pixel $t_n$ over each class. The adversarial attack aims to fool the model $f$ so that it predicts wrong label for all pixels
% {\em i.e.}, $\forall n$, ${\arg\max_c\left\{f_c\!\left(\mathbf{X}+\mathbf{r},t_n\right)\right\}}\neq{l_n}$. To achieve this goal, the algorithm crafts a wrong label set by randomly sampled from incorrect classes, which is denoted as ${\mathcal{L}'}={\left\{l'_1,l'_2,\ldots,l'_n\right\}}$, where $\forall i, l_i \neq l'_i$ The algorithm then minimize the loss $L$ that drive each every pixel to be incorrectly predicted ({\em i.e.}, suppressing the confidence of the original correct class $f_{l_n}\!\left(\mathbf{X}+\mathrm{r},t_n\right)$,
% while increasing  the confidence of desired (adversarial) incorrect class $f_{l'_n}\!\left(\mathbf{X}+\mathrm{r},t_n\right)$)

% \begin{equation}
% \label{Eqn:LossFunction}
% {L\!\left(\mathbf{X},\mathcal{T},\mathcal{L},\mathcal{L}'\right)}=
%     {{\sum_{n=1}^N}\left[{f}_{l_n}\!\left(\mathbf{X},t_n\right)-{f}_{l_n'}\!\left(\mathbf{X},t_n\right)\right]}
% \end{equation}



% \setlength{\algomargin}{0.5em}
% %\SetAlgoNlRelativeSize{0.1}
% \SetNlSkip{0.4em}
% \SetNlSty{text}{}{}
% \begin{algorithm}[t!]
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \SetKwInOut{Return}{Return}
% \Input{
%     input image $\mathbf{X}$;\\
%     \ the classifier ${\mathbf{f}\!\left(\cdot,\cdot\right)}\in{\mathbb{R}^C}$;\\
%     \ the target set ${\mathcal{T}}={\left\{t_1,t_2,\ldots,t_N\right\}}$;\\
%     \ the original label set ${\mathcal{L}}={\left\{l_1,l_2,\ldots,l_N\right\}}$;\\
%     \ the adversarial label set ${\mathcal{L}'}={\left\{l'_1,l'_2,\ldots,l'_N\right\}}$;\\
%     \ the maximal iterations $M_0$;
% }
% \Output{
%     the adversarial perturbation $\mathbf{r}$;
% }
% ${\mathbf{X}_0}\leftarrow{\mathbf{X}}$, ${\mathbf{r}}\leftarrow{\mathbf{0}}$,
% %${M}\leftarrow{0}$, ${\mathcal{T}_0}={\left\{1,2,...,N\right\}}$;\\ ZHISHUAI
% ${m}\leftarrow{0}$, ${\mathcal{T}_0}\leftarrow\mathcal{T}$;\\ % ZHISHUAI
% \While{${m}<{M_0}$ {\bf and} ${\mathcal{T}_m}\neq{\varnothing}$}{
%     ${\mathcal{T}_m}={\left\{t_n\mid\arg\max_c\left\{f_c\!\left(\mathbf{X}_m,t_n\right)\right\} = l_n\right\}}$;\\
% %    ${\mathbf{r}_m}\leftarrow{{\sum_{n\in\mathcal{T}_m}} ZHISHUAI
%     ${\mathbf{r}_m}\leftarrow{{\sum_{t_n\in\mathcal{T}_m}} %ZHISHUAI
%         \left[\nabla_{\mathbf{X}_m}f_{l'_n}\!\left(\mathbf{X}_m,t_n\right)-
%         \nabla_{\mathbf{X}_m}f_{l_n}\!\left(\mathbf{X}_m,t_n\right)\right]}$;\\
%     ${\mathbf{r}'_m}\leftarrow{\frac{\gamma}{\left\|\mathbf{r}_m\right\|_\infty}\mathbf{r}_m}$;\\
%     ${\mathbf{r}}\leftarrow{\mathbf{r}+\mathbf{r}'_m}$;\\
% %    ${\mathcal{T}_m}={\left\{n\mid\arg\max_c\left\{f_c\!\left(\mathbf{X}_m,t_n\right)\right\} = l_n\right\}}$;\\ ZHISHUAI
%     ${\mathbf{X}_{m+1}}\leftarrow{\mathbf{X}_m+\mathbf{r}'_m}$;\\
%     ${m}\leftarrow{m+1}$;
% }
% \Return{
%     $\mathbf{r}$
% }
% \caption{
%     Dense Adversary Generation (DAG)
% }
% \label{Alg:DAG}
% \end{algorithm}
\end{enumerate}

==> supp_supper_white.tex <==
\begin{table*}[h]
	% \begin{center}
		\vspace{-2mm}
		\begin{minipage}{0.71\linewidth}
			\begin{adjustbox}{width=1.4\linewidth}
				{\small
					\addtolength{\tabcolsep}{0pt}
					% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
					\begin{tabular}{l|ccccccccccc}
						\hline
						\hline
						 & \multicolumn{2}{c}{Super-FSGM} & \multicolumn{2}{c}{Super-PGD} & \multicolumn{2}{c}{Super-BIM} & \multicolumn{2}{c}{Super-DeepFool} & \multicolumn{2}{c}{Super-C\&W}  & Super-NewtonFool\\
						 & $2/255\uparrow$ & $4/255\uparrow$ &$2/255\uparrow$ & $4/255\uparrow$ & $2/255\uparrow$ & $4/255\uparrow$ & $L_{\infty}\uparrow$ & $L_{2}\uparrow$ & $L_{\infty}\uparrow$ & $L_{2}\uparrow$  &  $L_{\infty}\uparrow$
						 \\ 
						 \hline
						% \hline
						ComDefend\cite{jia2019comdefend} & 7.43 & 5.12&	1.33 & 0.80 &	1.54 &  0.82  &	1.83 & 1.70 &	2.47 & 1.02 &	0.45
								\\			
						Proposed method w/ $G$ only  & 11.97 & 7.82&	3.68 & 1.83 &	4.02 &  2.35  &	3.27 & 2.11 &	4.93 & 1.36 &	0.83
								\\									
						% \hline
						Proposed Method   & \textbf{62.88} & \textbf{55.25}  & \textbf{65.05}  & \textbf{63.97} &	\textbf{64.49} & \textbf{60.56} &	\textbf{68.62} & \textbf{59.93} &	\textbf{68.74} & \textbf{65.13}  &	\textbf{38.41}
						\\
						\hline
						\hline
						  
					\end{tabular}\\
				}
			\end{adjustbox}
		\end{minipage}
		\vspace{2mm}
		 \large{ \caption{We evaluate the defense performance against a super-white attack setting, where we assume the preprocessing model is exposed and the adversary can calculate the gradient for the differentiable part of the preprocessing model to construct stronger adversarial attacks. In such a setting, the differentiable preprocessing module (\ie, ComDefend and $G$ only) fail while our method does not collapse, demonstrating the benefit of exploiting the conventional ISP operator $S$ in our method.}  \label{tbl:super-white}}
	% \end{center}
	\vspace{-8mm}
\end{table*}

We conduct a super-white attack experiment to provide insights into the benefits of the proposed non-differentiable $S$ operator. A white-box setting means the attack methods have full access to a target model, including network architecture,  learned weights, and even training data, yet not to the preprocessing module used to transform input. In contrast, in the super-white box attack setting, both preprocessing modules and target models are exposed, allowing the adversary to calculate the gradient for adversarial attacks. In Table~\ref{tbl:super-white}, we demonstrate the defense performances of three competing approaches on the ImageNet in Top-1 accuracy under the super-white box attack setting. We see that the defense methods with differentiable preprocessing modules (\ie, ComDefend and the proposed method with $G$ only) cannot function effectively under the super-white box attack setting. The attack only impacts the proposed method marginally, validating the benefit of the non-differentiable $S$ operator. 

% We compared our method with the learning-based ComDefend baseline, as well as our method that used Learned ISP $G$ only. As the experiment in table~\ref{tbl:super-white} shows, the differentiable preprocessing module would fail in the super white setting. This demonstrates the benefit of exploiting the conventional ISP operator $S$ in our method.

% When evaluating the performance of defense algorithm in a white-box setting, most defense papers assume the adversary has full access to the target model (i.g. ResNet classification model), yet not to the preprocessing module used to transform the input. This section considers the case where the preprocessing model is exposed and allows the adversary to calculate the gradient for the differentiable part of the preprocessing model to construct strong adversarial attacks. We refer to these attacks as super-white attacks. In Table~\ref{tbl:super-white}, we evaluate the defense performance of three competing approaches on the ImageNet in Top-1 accuracy under this super-white attack setting. Based on the insights, the differentiable preprocessing module (\ie, ComDefend and Ours w/ $G$ only) would fail in the super white setting. This demonstrates the benefit of exploiting the conventional ISP operator $S$ in our method. Although this case would require knowledge of the defense method, we evaluate the defense performance on ImageNet. 
% % Bo: the logic is not clear to me.

% We compared our method with the learning-based ComDefend baseline, as well as our method that used Learned ISP $G$ only. As the experiment in table~\ref{tbl:super-white} shows, the differentiable preprocessing module would fail in the super white setting. This demonstrates the benefit of exploiting the conventional ISP operator $S$ in our method.


